Small-world networks and RNA secondary structures

Let Sn denote the network of all RNA secondary structures of length n, in which undirected edges exist between structures s, t such that t is obtained from s by the addition, removal or shift of a single base pair. Using context-free grammars, generating functions and complex analysis, we show that the asymptotic average degree is O(n) and that the asymptotic clustering coeffcient is O(1/n), from which it follows that the family Sn, n = 1,2,3,... of secondary structure networks is not small-world.

==> figures.tex <==



%Figure 1
\begin{figure}
\centering
\includegraphics[width=\textwidth]{figure1}
\caption{{\em (a)} Consensus secondary structure of the type III 
hammerhead ribozyme from Peach Latent Mosaic Viroid (PLMVd) AJ005312.1/282-335
(isolate LS35, variant ls16b), taken from Rfam \cite{Gardner.nar11}
family RF00008. 
%This structure was obtained using {\tt RNAfold} from
%the Vienna RNA Package \cite{Lorenz.amb11} with Turner99 energy parameters.
%Minimum free energy structure
%computed by Vienna RNA Package {\tt RNAfold} \cite{Lorenz.amb11} using
%Turner99 energy parameters, displayed with color-coded positional entropy. 
{\em (b)} 
Network for size 7 homopolymer with $\theta=3$, having 8 nodes and 
8 red $MS_1$ edges (base pair addition or removal), 8 blue $MS_2-MS_1$
edges (base pair shift), hence
a total of 16 $MS_2$ edges. It follows that $MS_1$ degree is 
$\frac{16}{8}=2$, while MS2 is $\frac{32}{8}=4$. 
}
\label{fig:secStr}
\end{figure}


%Figure 2
\begin{figure}
\centering
\includegraphics[width=\textwidth]{figure2}
\caption{Illustration of possible shift moves, where each subcaption
indicates the terminal symbols involved in the corresponding production
rule.  Solid blue [resp. dashed green] lines indicate the initial 
[resp. final] base pair in a shift move.
}
\label{fig:shiftMoves}
\end{figure}




%Figure 3
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figure3}
\caption{(a) $MS_2$-degree distribution for the 106,633 secondary 
structures for a 
20-nt homopolymer with $\theta=3$ (green shaded curve), with Poisson
distribution of the same mean.
(b) Plot of $\ln(\mbox{density})$ as a function
of $\ln(\mbox{degree})$ for the degree distribution for $MS_2$
connectivity of the
20-nt homopolymer with $\theta=3$, for degrees $4,\ldots,136$.
The distribution tail appears to satisfy
a power-law with exponent $\approx -5.6247$, i.e.
$p(x) \propto  x^{-5.6247}$,
where $x$ is degree and $p(x)$ is the relative frequency of the number of
nodes having degree $x$ (regression equation for log-log plot is
$\ln(p(x)) = 14.7589 - 5.6247 \cdot x$).
}
\label{fig:degreeDist20mer}
\end{figure*}


